Scalable Comparative Visualization of Ensembles of Call Graphs

Optimizing the performance of large-scale parallel codes is critical for efficient utilization of computing resources. Code developers often explore various execution parameters, such as hardware configurations, system software choices, and application parameters, and are interested in detecting and understanding bottlenecks in different executions. They often collect hierarchical performance profiles represented as call graphs, which combine performance metrics with their execution contexts. The crucial task of exploring multiple call graphs together is tedious and challenging because of the many structural differences in the execution contexts and significant variability in the collected performance metrics (e.g., execution runtime). In this paper, we present an enhanced version of CallFlow to support the exploration of ensembles of call graphs using new types of visualizations, analysis, graph operations, and features. We introduce ensemble-Sankey, a new visual design that combines the strengths of resource-flow (Sankey) and box-plot visualization techniques. Whereas the resource-flow visualization can easily and intuitively describe the graphical nature of the call graph, the box plots overlaid on the nodes of Sankey convey the performance variability within the ensemble. Our interactive visual interface provides linked views to help explore ensembles of call graphs, e.g., by facilitating the analysis of structural differences, and identifying similar or distinct call graphs. We demonstrate the effectiveness and usefulness of our design through case studies on large-scale parallel codes.

==> 5_2_actions.tex <==
\para{Comparison actions} are visualization tasks needed
to understand the relationships between and within comparison
targets.
%
Formulation of actions highly influences the visual encoding and the user
interactions that link individual visual components. Visualization
of ensembles of call graphs broadly require six actions.

\para{A1. Compare calling contexts across runs.} Due to potential
differences in calling contexts of the different executions (\textbf{T1}), it is essential
to highlight any differences, \ie missing nodes/edges in the graph.

\para{A2. Compare performance variability across runs.}
Displaying the aggregated performance from individual executions is not a
scalable approach considering the effort from the user, and the corresponding
visualization complexity.
%
%To simplify this, CallFlow should not only aggregate the recorded performance
Instead, the recorded performance (\textbf{T1}) and
calling contexts (\textbf{T2}) must be summarized not only within a single
execution, but also across multiple call graphs.

% Since it is impractical to display aggregated performance metrics (\textbf{T2})
% from each execution individually, CallFlow should summarize both the performance
% data and the super graphs across multiple executions and simplify the user-effort.

\para{A3. Compare performance variability across MPI ranks.}
%To quantify load imbalances across executions, CallFlow demands richer set of
%information during the post-mortem analysis.
%
Summary statistics, \eg mean runtime, across MPI ranks (\textbf{T3}) is not sufficient
to analyze
%only provides a qualititative summary of the 
runtime distribution across resources because the distribution is not
expected to be normal.
%
To aid the exploration, complete distributions are essential to visualize.

% additional statistics from the data should be
%readily available on-demand, such as medians and standard deviations of the
%executions, as well as identification of outliers.
%

\para{A4. Compare call graphs across levels of detail.} Although
comparisons across super graphs (semantically aggregated call graphs)
is useful, experts typically identify problem areas and are interested in
looking it selected regions in more detail. There, it is important
to manage fine-level details and visualize them upon request.
%
%As discussed in \autoref{sec:data}, the $d_{i}$ comprises of multiple
%granularities -- \textit{module}, \textit{call site name}, and \textit{ranks}.
%%
%These granularities help relate the runtime performance (\textbf{T2}) to other
%dimensions of data while comparing super nodes for interesting behaviors.
%%
%Therefore, CallFlow should support runtime analysis against each granularity to
%help pinpoint interesting call sites.
%% It is thus crucial to compare the the targets against the granularities to help pinpoint to call sites that reveal interesting behaviors.
%% In future, many more data granularities that affect the performance could be introduced based on the kinds of experiment performed.
%%

\para{A5. Compare two call graphs.}
Differences between two call graph can exist structurally (\textbf{T1}), as
runtime variations (\textbf{T2, T3}), and/or in execution parameters (\textbf{T4}).
%
Simple, visual representations of such differences is of value to the user,
but can be visually overwhelming and computationally expensive
for comparison.

%%
%Therefore, CallFlow must distill out the structurally similar callsites and help
%focus on revealing callsites that exhibit high runtime variation.

\para{A6. Compare a selected run with an ensemble.}
Comparison tasks often require a {baseline} to compare against.
For all of our targets (\textbf{T1--T4}), it is important to
compare a selected run with the ensemble behavior.
%
An important constraint to consider is that the constructed baseline must match
the expert's understanding of the overall calling context, despite minor
differences in the individual ensemble members.

% To understand the evolution of the changes across experiments, scientists need
% to compare connectivity data gathered at different instances.
% %
% Therefore, it is required to develop mechanisms to find similar runs based on
% calling structure.


==> 5_5_interactions.tex <==
\subsubsection{Interactions Between Views}
\noindent\textbf{Revealing nodes in the ensemble-Sankey.}

1. using click interactions on the supernode hierarchy
2. additional flexibility for the user to choose the call sites that for various splitting operations.


\noindent\textbf{Selecting target and compare dataset.}
During comparative analysis, the user might find a particular execution or two that exhibit a variation in the ensemble distribution, or appear an outlier
from the projection view.
%
To allow the user select a run, and might want to compare the runs with respect to that run.
% %
% To support this, the user can right click on the circles in the projection view
% and the corresponding views are updated.

\noindent\textbf{Sorting using distribution statistics.}
Call sites in the correspondence view can be sorted based on various statistical measures like inclusive/exclusive runtime, median, or standard deviation. 

\noindent\textbf{Details on demand using tooltips.}
Hovering the mouse pointer for a few seconds over any part of the overview will display a tooltip, summarizing the information or values under the pointer.


%
% Available statistics include average, median, maximum,minimum, standard 
% deviation, variance, skewness, kurtosis and bimodality.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% Notes %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Read these
% 1. Scenario-Based Comparison of Clone Detection Techniques (For detecting similar CCTs)
% 2. A tree distance function based on multi-sets. (For distance metric that considers multi-sets of calling contexts.)
% 3.

==> __latexindent_temp.tex <==
Optimizing the performance of large-scale parallel codes is critical for
efficient utilization of computing resources. Code developers often explore
various execution parameters, such as hardware configurations, system software
choices, and application parameters, and are interested in detecting and
understanding bottlenecks in different executions.  They often collect
hierarchical performance profiles represented as call graphs, which combine
performance metrics with their execution contexts. 
The crucial task of exploring multiple call graphs together is tedious and
challenging because of the many structural differences in the execution
contexts and significant variability in the collected performance metrics (\eg
execution runtime). In this paper, we present an enhanced version of CallFlow
to support the exploration of ensembles of call graphs using new types of
visualizations, analysis, graph operations, and features.  We introduce
\emph{ensemble-Sankey}, a new visual design that combines the strengths of
resource-flow (Sankey) and box-plot visualization techniques.  Whereas the
resource-flow visualization can easily and intuitively describe the graphical
nature of the call graph, the box plots overlaid on the nodes of Sankey convey
the performance variability within the ensemble.
Our interactive visual interface provides linked views to help explore
ensembles of call graphs, \eg by facilitating the analysis of structural
differences, and identifying similar or distinct call graphs.We demonstrate the effectiveness and usefulness of our design through case
studies on large-scale parallel codes.
\vspace{-0.7em}


